Which Prompting Technique Should I Use? An Empirical Investigation of Prompting Techniques for Software Engineering Tasks

A growing variety of prompt engineering techniques has been proposed for Large Language Models (LLMs), yet systematic evaluation of each technique on individual software engineering (SE) tasks remains underexplored. In this study, we present a systematic evaluation of 14 established prompt techniques across 10 SE tasks using four LLM models. As identified in the prior literature, the selected prompting techniques span six core dimensions (Zero-Shot, Few-Shot, Thought Generation, Ensembling, Self-Criticism, and Decomposition). They are evaluated on tasks such as code generation, bug fixing, and code-oriented question answering, to name a few. Our results show which prompting techniques are most effective for SE tasks requiring complex logic and intensive reasoning versus those that rely more on contextual understanding and example-driven scenarios. We also analyze correlations between the linguistic characteristics of prompts and the factors that contribute to the effectiveness of prompting techniques in enhancing performance on SE tasks. Additionally, we report the time and token consumption for each prompting technique when applied to a specific task and model, offering guidance for practitioners in selecting the optimal prompting technique for their use cases.

==> tables/kappa_tables.tex <==


\begin{table}[h]
    \centering
    \small
    \caption{Cohen’s kappa result by Prompting Technique}
    \renewcommand{\arraystretch}{0.9} 
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{p{4cm} c c c}
        \toprule
        \textbf{Prompt Technique}    & \textbf{Po} & \textbf{Pe} & \textbf{k}  \\
        \midrule
        rephrase\_and\_respond       & 1,00        & 1,00        & ---         \\
        role\_prompting              & 0,81        & 0,81        & 0,00        \\
        emotion\_prompting           & 0,83        & 0,83        & 0,00        \\
        self\_ask                    & 1,00        & 0,99        & 1,00        \\
        tree\_of\_thought            & 1,00        & 0,97        & 1,00        \\
        universal\_self\_consistency & 1,00        & 0,96        & 1,00        \\
        style\_prompting             & 0,98        & 0,85        & 0,87        \\
        exemplar\_selection\_knn     & 1,00        & 1,00        & ---         \\
        few\_shot\_contrastive\_cot  & 1,00        & 1,00        & ---         \\
        self\_refine                 & 0,94        & 0,85        & 0,61        \\
        sg\_in\_context\_learning    & 0,91        & 0,86        & 0,33        \\
        thread\_of\_thought          & 1,00        & 0,85        & 1,00        \\
        step\_back\_prompting        & 0,89        & 0,87        & 0,18        \\
        analogical\_prompting        & 0,98        & 0,92        & 0,76        \\
        \bottomrule
    \end{tabular}
    
    \label{tab:kappa_techniques}
\end{table}

\begin{table}[h]
    \centering
    \small
    \caption{Cohen’s kappa result by SE Task}
    \renewcommand{\arraystretch}{0.9} 
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{p{4cm} c c c}
        \toprule
        \textbf{Task}      & \textbf{Po} & \textbf{Pe} & \textbf{k} \\
        \midrule
        Assert Generation  & 0,95        & 0,89        & 0,53       \\
        Code Summarization & 0,92        & 0,89        & 0,29       \\
        Clone Detection    & 0,95        & 0,90        & 0,45       \\
        Defect Detection   & 0,95        & 0,88        & 0,57       \\
        Bug Fixing         & 0,99        & 0,94        & 0,76       \\
        Code Translation   & 0,97        & 0,94        & 0,44       \\
        Code Generation    & 0,96        & 0,92        & 0,54       \\
        Exception Type     & 0,93        & 0,90        & 0,26       \\
        Code QA            & 0,96        & 0,96        & -0,02      \\
        Mutant Generation  & 0,97        & 0,90        & 0,68       \\ 
        \bottomrule
    \end{tabular}
    
    \label{tab:kappa_tasks}
\end{table}



==> tables/rq2_correlations_report.tex <==
\begin{table}
\centering
\footnotesize
\caption{Correlation between prompt performance and different textual metrics}
\label{tab:correlations_with_text_metrics}
\begin{tabular}{p{2.5cm}lccccc}
\toprule
Groups & Test & p\_value & corr\_coef \\
\midrule
code\_generation & mean\_gunning\_fog & 0.0012 & -0.3364 \\
code\_understanding & mean\_mtld & 0.0048 & -0.3591 \\
code\_understanding & mean\_fk\_grade & 0.0215 & 0.2964 \\
code\_understanding & mean\_gunning\_fog & 0.0139 & 0.3160 \\
code\_understanding & mean\_flesch\_reading\_ease & 0.0020 & -0.3906 \\
global\_aggregate & mean\_prompt\_time & 0.0490 & -0.1610 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/rq3_aggregate_technique_performance.tex <==
\begin{table*}
\centering
\footnotesize
\caption{Aggregate comparison to token and time cost-benefit performance}
\label{aggregate_performance_data}
\begin{tabular}{lccccc}
\toprule
Task\_name & Scenario & std\_dev & Best\_technique\_name & Best\_metric\_result & Control\_result & Worst\_technique\_name & Worst\_metric\_result \\
\midrule
Defect detection & Performance & 3.60 & ToT & 73.66 & 66.22 & SR & 59.91 \\
Defect detection & Performance/Token & 0.07 & RP & 0.19 & 0.22 & ES-KNN & 0.03 \\
Defect detection & Performance/Time & 7.61 & ES-KNN & 25.32 & 23.52 & USC & 0.75 \\
Clone detection & Performance & 1.17 & ES-KNN & 68.60 & 66.03 & SG-ICL & 63.45 \\
Clone detection & Performance/Token & 0.03 & SP & 0.10 & 0.09 & ES-KNN & 0.02 \\
Clone detection & Performance/Time & 6.16 & ES-KNN & 21.20 & 20.08 & USC & 1.24 \\
Exception type & Performance & 7.16 & ES-KNN & 82.50 & 78.16 & ToT & 52.04 \\
Exception type & Performance/Token & 0.06 & RP & 0.20 & 0.22 & ES-KNN & 0.04 \\
Exception type & Performance/Time & 7.62 & ES-KNN & 27.68 & 23.23 & USC & 1.84 \\
Code QA & Performance & 1.39 & USC & 55.67 & 50.99 & TroT & 51.44 \\
Code QA & Performance/Token & 0.07 & RP & 0.25 & 0.28 & TroT & 0.02 \\
Code QA & Performance/Time & 5.15 & ES-KNN & 19.23 & 16.57 & USC & 0.92 \\
\textbf{Code understanding group} & Performance & 2.15 & ES-KNN & 69.27 & 65.35 & ToT & 60.87 \\
\textbf{Code understanding group} & Performance/Token & 0.05 & RP & 0.18 & 0.20 & SR & 0.03 \\
\textbf{Code understanding group} & Performance/Time & 6.48 & ES-KNN & 23.36 & 20.85 & USC & 1.19 \\
Code translation & Performance & 6.30 & ES-KNN & 42.08 & 30.19 & TroT & 13.39 \\
Code translation & Performance/Token & 0.06 & RP & 0.17 & 0.19 & USC & 0.01 \\
Code translation & Performance/Time & 3.20 & ES-KNN & 11.53 & 7.18 & USC & 0.33 \\
Bug fixing & Performance & 4.69 & SG-ICL & 36.02 & 36.26 & TroT & 16.45 \\
Bug fixing & Performance/Token & 0.05 & RP & 0.15 & 0.18 & USC & 0.00 \\
Bug fixing & Performance/Time & 2.42 & ES-KNN & 8.93 & 7.58 & USC & 0.22 \\
Mutant generation & Performance & 19.59 & ES-KNN & 69.93 & 67.98 & TroT & 16.44 \\
Mutant generation & Performance/Token & 0.12 & RP & 0.35 & 0.37 & USC & 0.01 \\
Mutant generation & Performance/Time & 5.87 & ES-KNN & 20.16 & 15.21 & USC & 0.28 \\
Assert generation & Performance & 15.23 & ES-KNN & 65.44 & 25.24 & TroT & 0.92 \\
Assert generation & Performance/Token & 0.02 & RP & 0.04 & 0.05 & TroT & 0.00 \\
Assert generation & Performance/Time & 5.27 & ES-KNN & 20.88 & 6.84 & USC & 0.07 \\
Code summarization & Performance & 1.51 & SG-ICL & 4.15 & 4.16 & ToT & 0.45 \\
Code summarization & Performance/Token & 0.01 & RP & 0.02 & 0.02 & USC & 0.00 \\
Code summarization & Performance/Time & 0.28 & ES-KNN & 0.61 & 1.02 & USC & 0.02 \\
Code generation & Performance & 3.04 & USC & 24.44 & 23.18 & TroT & 13.45 \\
Code generation & Performance/Token & 0.01 & SA & 0.03 & 0.03 & USC & 0.00 \\
Code generation & Performance/Time & 1.02 & ES-KNN & 4.39 & 1.81 & USC & 0.14 \\
\textbf{Code generation group} & Performance & 6.83 & ES-KNN & 38.55 & 31.17 & TroT & 10.32 \\
\textbf{Code generation group} & Performance/Token & 0.04 & RP & 0.13 & 0.14 & USC & 0.00 \\
\textbf{Code generation group} & Performance/Time & 2.88 & ES-KNN & 11.08 & 6.61 & USC & 0.18 \\
\bottomrule
\end{tabular}
\end{table*}

